Combining ID's, Attributes, and Policies in Hyperledger Fabric

This work aims to provide a more secure access control in Hyperledger Fabric blockchain by combining multiple ID's, attributes, and policies with the components that regulate access control. The access control system currently used by Hyperledger Fabric is first completely analyzed. Next, a new implementation is proposed that builds upon the existing solution but provides users and developers with easier ways to make access control decisions based on combinations of multiple ID's, attributes, and policies. Our proposed implementation encapsulates the Fabric CA client to facilitate attribute addition and simplify the process of registering and enrolling a newly created certificate (corresponding to a new user). This research, concludes that it is possible to combine multiple ID's, attributes, and policies with the help of Hyperledger Fabric's smart contract technology. Furthermore, it could be seen that the performance impact for real-world applications is negligible compared to the insecure case of always providing access to a resource without performing access control.

==> sections/responsible_research.tex <==
\section{Responsible Research}
This section will reflect on the ethical aspects and the reproducibility of the study performed in this research paper.

\subsection{Ethical Aspects}
As described in Section 1, this study aims to present a way to provide secure access control by combining multiple ID's, attributes, and policies within Hyperledger Fabric blockchain networks. As a result, the most important ethical aspects relevant to this study are the security and privacy of the Hyperledger Fabric blockchain technology. While most traditional blockchain technologies do not provide ways to easily establish privacy and trust on the network, Hyperledger Fabric enables blockchain participants to identify each other through the use of identities. In addition, Hyperledger Fabric allows users to protect their data from other blockchain participants through the use of channels and private data collections. Because of these innovative techniques, Hyperledger Fabric provides all the basic features that traditional blockchains can offer, and builds upon these features to offer trust and privacy on the blockchain network.

An important point in the context of ethical responsibility is that this research aims to contribute to the security of Hyperledger Fabric by improving its access control mechanism. While access control must currently be performed by validating individual X.509 certificates within smart contracts, the solutions proposed in this paper allow smart contract developers to easily combine multiple ID's, attributes, and policies during their access control decisions. This allows smart contracts to make more fine-grained access control decisions, which in turn makes it easier to adhere to the principle of least privilege \cite{least-privilege}. Therefore, the contributions of this paper only aim to improve the security and privacy of Hyperledger Fabric and can thus be considered ethically responsible. 

\subsection{Reproducibility}
It is highly important that research is conducted in such a way that it is reproducible. By allowing other researchers to repeat the study presented in this paper, all contributions and results can objectively be validated. To guarantee the reproducibility of this particular study, several measures have been taken. First, Section 3 of this paper aims to provide an in-depth explanation of the methodology that was used to arrive at the final contributions. Second, the entire code-base that has been implemented as part of this study has been made publicly available on GitHub\cref{github-repository}. Finally, Section 6 presents the raw benchmark data that has been obtained, which can also be found in the \texttt{README} file inside the \texttt{caliper} directory of the aforementioned GitHub repository. Thus, since all research data is made publicly available, this study should be fully reproducible by other researchers.
